Causal Inference in Observational Studies with Non-Binary Treatments

Propensity score methods have become a part of the standard toolkit for applied researchers who wish to ascertain causal effects from observational data. While they were originally developed for binary treatments, several researchers have proposed generalizations of the propensity score methodology for non-binary treatment regimes. Such extensions have widened the applicability of propensity score methods and are indeed becoming increasingly popular themselves. In this article, we closely examine the two main generalizations of propensity score methods, namely, the propensity function (P-FUNCTION) of Imai and van Dyk (2004) and the generalized propensity score (GPS) of Hirano and Imbens (2004), along with recent extensions of the GPS that aim to improve its robustness. We compare the assumptions, theoretical properties, and empirical performance of these alternative methodologies. On a theoretical level, the GPS and its extensions are advantageous in that they can be used to estimate the full dose response function rather than the simple average treatment effect that is typically estimated with the P-FUNCTION. Unfortunately, our analysis shows that in practice response models often used with the original GPS are less flexible than those typically used with propensity score methods and are prone to misspecification. We compare new and existing methods that improve the robustness of the GPS and propose methods that use the P-FUNCTION to estimate the dose response function. We illustrate our findings and proposals through simulation studies, including one based on an empirical application.

==> deleted_sections <==
\subsection{Simulation study III}
\label{sec:sim-three}

Simulation I and II assume a correctly specified treatment model. To investigate
the effect of treatment model misspecification, we extend a simulation study
from \citet{kang:scha:07} into the continuous treatment case. In particular, for
each unit $i=1,\ldots,2000,$ we generate $(Z_{i1},Z_{i2},Z_{i3},Z_{i4})^T$
independently from $N(0,I)$ where $I$ is the identity matrix, set
\[
Y_i = 210+27.4Z_{i1}+13.7Z_{i2}+13.7Z_{i3}+13.7Z_{i4}+\epsilon_i,
\]
where $\epsilon_i \sim N(0,1)$, and set
\[
T_i = -Z_{i1}+0.5Z_{i2}-0.25Z_{i3}-0.1Z_{i4}+\sigma_i,
\]
where $\sigma_i \sim N(0,1)$. In our analysis, however, we assume that we
observe $X_{i1} = \exp(Z_{i1}/2)$, $X_{i2} = Z_{i2}/(1+\exp(Z_{i1})) + 10$,
$X_{i3} = (Z_{i1}Z_{i3}/25+0.6)^3$, and $X_{i4} = (Z_{i2}+Z_{i4}+20)^2$, rather
than the $Z_{ij}$'s. The diagnostic tools introduced in
Section~\ref{sec:gen_pscore} did not detect this missepcification.

The estimated relative \drfs~from the \hi, \scm(\gps), \scm(\pfun), and
\iw~methods are shown in Figure~\ref{fig:sim_III} .
Apart from \iw, which again shows significantly larger standard deviation than
the others methods\footnote{For the IW method under the wrong treatment model,
18 out of the 1000 replications led to numerical instability. The plotted result
is based on the remaining 982 replications.}, only the two standard deviation
intervals under the \scm(\pfun) method cover the true relative \drf. Both
the \hi~and \scm(\gps) methods show a cyclic bias.


\begin{figure}
\spacingset{1}
\centering
\textsf{\textbf{\large Using the Correct Treatment Model}}\\ \smallskip
\includegraphics[width=0.24\textwidth]{Figs/Sim_III/true_trt_model/hi_dr.pdf}
\includegraphics[width=0.24\textwidth]{Figs/Sim_III/true_trt_model/scm_gps_dr.pdf}
\includegraphics[width=0.24\textwidth]{Figs/Sim_III/true_trt_model/scm_pfunc_dr.pdf}
\includegraphics[width=0.24\textwidth]{Figs/Sim_III/true_trt_model/iw_dr.pdf}
\textsf{\textbf{\large Using the Wrong Treatment Model}}\\ \smallskip
\includegraphics[width=0.24\textwidth]{Figs/Sim_III/wrong_trt_model/hi_dr.pdf}
\includegraphics[width=0.24\textwidth]{Figs/Sim_III/wrong_trt_model/scm_gps_dr.pdf}
\includegraphics[width=0.24\textwidth]{Figs/Sim_III/wrong_trt_model/scm_pfunc_dr.pdf}
\includegraphics[width=0.24\textwidth]{Figs/Sim_III/wrong_trt_model/iw_dr.pdf}  
\caption{{\bf Estimated Relative \drf\ in Simulation III. The first row is
fitted using the correct treatment model while the second row is fitted using
the wrong treatment model. In all plots solid lines represent the true
  relative \drfs\ while dashed lines represent the means of the fitted relative
  \drfs\ across the 1000 simulations. The gray shaded regions correspond to two
  standard deviation pointwise intervals across the 1000 fitted relative \drfs.
  The evenly-spaced grid of evaluation points are identical for all plots
  and plotted as solid circles. Note that the scale of the y-axis for the method
  of IW under the wrong treatment model is much larger than the others as it
  has significantly larger standard deviation.}}
\label{fig:sim_III} 
\end{figure}  


#######################
#####  Section 3.3
#######################
In practice, the particular response models suggested by \ivd\ --
linear models within multiple subclasses and the \scm\ -- are more
flexible than the quadratic regression model suggested by \hi. In
Simulation study~II of Section~\ref{sec:sim-two}, for example, using a
linear model within each of ten classes involves fitting twenty mean
parameters and ten variance parameters, whereas the model suggested by
\hi\ has only six mean parameters and one variance parameter.  The
\scm\ given in equation~\eqref{eq:IvD-smooth-coef} is also very
flexible. If we constrain it so that $f$ is quadratic and $g$ is
linear, for example, the model reduces to the quadratic regression in
equation~\eqref{eq:gps-r-model} minus the $T^2$ term.  The full \scm\
is much more flexible than this. {\bf Besides, the \scm(\gps) method, which
replaces (\ref{eq:gps-r-model}) with a nonparametric model, doesn't perform well
in Simulation I either (see Figure~\ref{fig:sim1-1}). A tentative explanation is
offered in the Appendix.}

#########################
#### my explanation of SCM(GPS) failure
#########################
To visualize the distribution of the \gps~for one replicated data set, we
present two scatterplots of $Y$ and $T$ in Figure~\ref{fig:sim-four-color}. The
left plot points is color-coded based on $\hat R_i$ and the right plot is
color-coded based on $\hat{r}(t=-1,X_i)$. In both plots bluer (redder) points 
represent larger (smaller) value. The two clusters correspond to
$Z_i=0$ and $Z_i=1$.

The left plot illustrates why the response model of a \gps-based method does not
carry a causal interpretation. \gps\ response models condition on observed
treatment and the color in the left plot, where red represents more extreme
treatments given the covariates value and blue more likely treatments. To
estimate  the \drf\ at a given treatment level, say $t=-1$, \gps-based methods
use $\hat{r}(t=-1,X_i)$ to estimate the response of 
each observation if it had a treatment of $-1$.
Judging from the right panel of Figure~\ref{fig:sim-four-color}, most of the 
cluster corresponding to $Z_i=0$ is made up of units with a likely or very
likely treatment, while the $Z_i=1$ cluster is made of units with unlikely
treatments. Averaging over the entire sample thus give us an estimate of the \drf~at treatment level $t=-1$.

The problem, however, is the response model for the \scm(\gps)~method. Think
of $Z$ as the gender indicator variable, $X$ certain intermediate covariate
correlated to gender like weight, $T$ the amount of daily cigaratte usage, and $Y$ a health
status indicator variable. The setup is then to study the influence of smoking
on health. The response model, however, will classify the extreme smoker
and extreme nonsmoker for both male and female in the same sudo-subpopulation
(like those red points in the left plot of Figure~(\ref{fig:sim-four-color})).
It seems difficult, even with nonparametric technique, to find the correct
specification of such response model, if it exists.

{\bf SZ: delete this paragraph?} The right plot illustrates the weak
ignorability of the treatment assignment given the \gps. {\bf Explain here !!!} Now because $Z$ is the only variable that
influences $Y$, some function of $\hat R$ and $T$ must identify $Z$ for
\scm(\gps) to work. Unfortunately, the left plot illustrates that the
distributions of $\hat{R}$ are almost identical in the two clusters. It is
difficult to imagine any response model based on the \gps~that can deliver an
unbiased estimate of the \drf~in this simple setting. {\bf SZ: I don't think
this argument is strong as HI has stated their response model doesn't have
causal intrepretation.}

